Generative Induction of Dialogue Task Schemas with Streaming Refinement and Simulated Interactions

In task-oriented dialogue (TOD) systems, Slot Schema Induction (SSI) is essential for automatically identifying key information slots from dialogue data without manual intervention. This paper presents a novel state-of-the-art (SoTA) approach that formulates SSI as a text generation task, where a language model incrementally constructs and refines a slot schema over a stream of dialogue data. To develop this approach, we present a fully automatic LLM-based TOD simulation method that creates data with high-quality state labels for novel task domains. Furthermore, we identify issues in SSI evaluation due to data leakage and poor metric alignment with human judgment. We resolve these by creating new evaluation data using our simulation method with human guidance and correction, as well as designing improved evaluation metrics. These contributions establish a foundation for future SSI research and advance the SoTA in dialogue understanding and system development.

==> tex/misc/related-work-extra.tex <==

\paragraph{Event Schema Induction}
Inducing events, their arguments, and their relations from a corpus of documents is another popular area of study for schema induction work, with early works focusing on statistical techniques for unsupervised induction \cite{chambers-jurafsky-2008-unsupervised, chambers-jurafsky-2009-unsupervised, peng-etal-2016-event} and recent works leveraging LLMs in a question-answering formulation \cite{du-cardie-2020-eventqa, li-etal-2020-eventqa, lyu-etal-2021-eventqa, dror-etal-2023-zero}. Most similar to our work, recent approaches to event schema induction leverage LLMs for both synthetic data generation and subsequent schema induction \cite{dror-etal-2023-zero, zhang-etal-2023-human}, with some exploring iterative revision techniques although only human-in-the-loop revision techniques have been used to date \cite{zhang-etal-2023-human, mondal-etal-2025-adaptive}.

\citet{dror-etal-2023-zero} use GPT3 to generate synthetic information documents (how-to guide, news article, etc.) for given event descriptions, and then use traditional NLP tools (SRL, NER, relation extraction) to extract and organize pertinent information values about the described events and subevents. Using frequency statistics from a corpus, an event schema is induced from the extracted information, covering all events, their arguments, and relations.
Some works approach the task of event schema induction allowing for iterative revisions to the induced schema, although only human-in-the-loop revision techniques have been used to date. \citet{zhang-etal-2023-human} propose a four-stage schema induction system, in which GPT3 and a human collaborate to identify subevents of a high-level target event description, argument identification of subevents, event relation graph construction, and event grounding, resulting in a schema representation of each target event.
\citet{mondal-etal-2025-adaptive} use LLMs to predict relevant questions to represent the event information in a document corpus and embedding-based clustering techniques to group questions into slots and domains; the clusters are then iteratively refined using human feedback in the form of question-cluster constraints and subsequent embedding similarity procedures, until the human determines the induced schema is adequate.

\paragraph{Dialogue Flow Induction}
The goal of dialogue flow induction work is to extract general dialogue action workflows that consist of sequences of actions and slots necessary for accomplishing a specific dialogue goal. Most work in this area focuses on the induction of a dialogue flow for a single dialogue at a time \cite{el2023workflow} using text generation modeling in which the dialogue and action candidates are given as input and the workflow is given as output. \citet{burdisso-etal-2024-dialog2flow} propose a new utterance encoding strategy to improve clustering of utterances for dialogue flow induction.

Recently, \cite{choubey2025turning} extend dialogue flow induction to induce a general flow schema that represents dialogue flows over a corpus of dialogues. They use GPT4o-mini to extract intents, slot-values, and agent actions from a dialogue corpus, and use embedding representations of this extracted information to cluster dialogues with similar underlying goals together. These clustered dialogues are then processed through a question-answering LLM-to-LLM method and LLM aggregation method that together aim to extract a general dialogue workflow that represents the dialogues in the cluster. 




%%%%% not really slot schema due to bad setup
\citet{wu-active-discovering-2024} frame slot induction as a sequence labelling task and utilize active learning to elicit human annotations for value candidates with low-certainty labels to update the training dataset of the sequence labeler in an iterative fashion.






\paragraph{Dialogue State Tracking}
Current state-of-the-art (SoTA) approaches to zero-shot DST use sequence-to-sequence (S2S) modeling to predict appropriate values given a natural language specification of each slot to track \cite{gupta_show_2022, king_diverse_2023}. Such S2S modeling has been effective for adapting to new slot types, since models can leverage descriptions of a new, unseen slot type via in-context learning (ICL) when making predictions. Recently, models using LLMs have achieved state-of-the-art results on this task due to the excellent zero-shot ability of LLMs \cite{hu_-context_2022, king_diverse_2023}. However, the cost of LLM decoding is often too steep for many task-oriented dialogue (TOD) applications. Thus, ongoing work aims to achieve SoTA results with smaller models using cross-task transfer, where the model is trained on an existing set of task domains before being transferred to the unseen target domain \cite{wang_divide_2023, aksu_prompter_2023}.

